On sub-graphs of the Johnson $\mathcal{J}(n,k)$ graph induced by particle systems on simple graphs

Understanding the topology of the state space has proven to be extremely efficient for dynamical systems with a continuous state space. On the other hand, for particle systems on finite simple graphs, it has not yet been subject to deep investigation due to combinatorial hurdles and existing efficient spectral theoretic approaches to the analysis of classical particle systems. In the context of complex systems with heterogeneous interactions of particles, these techniques can break down due to intractability. This work provides a tool box of results on the topology of state spaces of particles systems under the sole conditions that exactly one particle moves at a time and no two particles may occupy the same vertex at the same time. The Johnson $\mathcal{J}(n,k)$ graph yields the overarching structure and we prove that any particle system with exclusion property and single particle movements may be embedded as a dynamical system on a sub-graph of $\mathcal{J}(n,k)$.

==> chapters/SNMaEP_IAE.tex <==
In this section we are going to establish basic properties of $\mathfrak{S}_k$ independent of the graph structure as long as $L$ is a connected simple graph. 
\vspace{5pt}
\begin{tcolorbox}[boxsep=0pt,arc=0pt,colback=burgundy!15!white, frame empty]%%
	\begin{theorem}\label{thm:S_irred_aperiodic}
 		The Markov chain $\mathfrak{S}_k$ on $\mathfrak{L}_k$ is irreducible and aperiodic. 
 	\end{theorem}
 \end{tcolorbox}
 	\begin{proof}
 		Let $\mathfrak{v},\mathfrak{w}\in \mathfrak{V}_k$ such that $p_{k;\mathfrak{v},\mathfrak{w}}^{\triangle}>0$. Then also $p_{k;\mathfrak{w},\mathfrak{v}}^{\triangle}>0$ even though equality is not necessarily satisfied. Furthermore every $\langle \mathfrak{w},\mathfrak{v}\rangle\in \mathfrak{E}_k$ implies that $p_{k;\mathfrak{v},\mathfrak{w}}^{\triangle}>0$. Since $\mathfrak{L}_k$ is connected by Proposition \ref{prop:L_frak_k_connected} we obtain that the chain is irreducible.\\ 
 		The aperiodicity of $\mathfrak{S}_k$ follows directly from the fact that we can construct a state $\mathfrak{v}\in \mathfrak{V}_k$ such that $p_{k;\mathfrak{v},\mathfrak{v}}^{\triangle}>0$.
 	\end{proof}
By Theorem \ref{thm:convergence_to_stat_dist_irred_aperiod} on Markov chains on finite state spaces, we can conclude from Theorem \ref{thm:S_irred_aperiodic} that $\mathfrak{S}_k$ is ergodic, i.e., there is a stationary distribution and the chain converges independently of its initial distribution to said stationary distribution. 
\vspace{5pt}
\begin{tcolorbox}[boxsep=0pt,arc=0pt,colback=burgundy!15!white, frame empty]%%
	\begin{theorem}\label{thm:S_existence_stat_dist}
 		Let $L=(V,E)$ be a $\bar{d}$-regular graph, $\bar{n}:=|V|$ and $k\in\{1,\hdots,\bar{n}-1\}$. Let $\mathfrak{L}_k=(\mathfrak{V}_k, \mathfrak{E}_k)$ be defined as in Definition \ref{def:mathfrak_L_k}. Then there exists a distribution $\tilde{\pi}_k$ on $\mathfrak{V}_k$ such that the Markov chain $\mathfrak{S}_k$ converges in distribution to $\tilde{\pi}_k$ independently of its initial distribution $\nu_0$. 
 	\end{theorem}
\end{tcolorbox}
Having found an answer to this classical question we can wonder about the structure of $\tilde{\pi}_k$ as a function of $L$ and other properties of $\mathfrak{S}_k$ which govern the long-time behavior, like reversibility. While the classical exclusion process is always reversible, it turns out the choice exclusion process implies a structure on the transition matrix of $\mathfrak{S}_k$ which is only reversible in rare cases. The echo chamber model, therefore, gives rise to a qualitatively different kind of exclusion process as has been investigated before. 
\subsubsection{Lumpability and isomorph bipartite sub-graphs}\label{subsubsec:lumpability_isom}
In this subsection we are going to develop the idea of lumping the state space in detail, as defined in Definition \ref{def:lumpability_markov_chains} Due to the sensitivity of the Markov chain $\mathfrak{S}_k$ with respect to the number of particles as well as the geometry of the underlying graph, we have to apply sensitive tools based on as much information as possible from each sub-graph induced by a set of particles $\mathfrak{v}\in\mathfrak{V}_k$. It turns out that the bipartite sub-graphs $L_{\mathfrak{v},\mathfrak{v}^c}$ play an essential role. In fact, they provide a stronger form of lumpability for $\mathfrak{S}_k$ when lumping with respect to the degree of $\mathfrak{v}$ in $\mathfrak{L}_k$ is not possible, i.e., in almost all non-reversible cases.
\vspace{5pt}
\begin{tcolorbox}[boxsep=0pt,arc=0pt,colback=burntorange!25!white, frame empty]%%
	\begin{proposition}\label{prop:isom_of_bipartites_implies_same_transition_vect}
		Let $k\in\left\{1,\hdots,\bar{n}-1\right\}$ and let $\mathfrak{v}, \mathfrak{w} \in \mathfrak{V}_k$. Consider the by decreasing size ordered vectors $(p^{\triangle}_{k;\mathfrak{v},\mathfrak{u}})_{\mathfrak{u}\in\mathfrak{V}_k}$, $(p^{\triangle}_{k;\mathfrak{w},\mathfrak{u}})_{\mathfrak{u}\in\mathfrak{V}_k}$, $(p^{\triangle}_{k;\mathfrak{u},\mathfrak{v}})_{\mathfrak{u}\in\mathfrak{V}_k}$ and $(p^{\triangle}_{k;\mathfrak{u},\mathfrak{w}})_{\mathfrak{u}\in\mathfrak{V}_k}$. Then, $L_{\mathfrak{v},\mathfrak{v}^c}\stackrel{\sim}{=} L_{\mathfrak{w},\mathfrak{w}^c}$ if and only if these vectors satisfy the identities
		\begin{align*}
			(p^{\triangle}_{k;\mathfrak{v},\mathfrak{u}})_{\mathfrak{u}\in\mathfrak{V}_k}=(p^{\triangle}_{k;\mathfrak{w},\mathfrak{u}})_{\mathfrak{u}\in\mathfrak{V}_k}\\
			(p^{\triangle}_{k;\mathfrak{u},\mathfrak{v}})_{\mathfrak{u}\in\mathfrak{V}_k}=(p^{\triangle}_{k;\mathfrak{u},\mathfrak{w}})_{\mathfrak{u}\in\mathfrak{V}_k}.
		\end{align*}
	\end{proposition}
\end{tcolorbox}
\begin{proof}
	The claim follows since the bipartite graphs are isomorphic and, hence, any transition from or to $\mathfrak{v}$, defined by an edge from $\mathfrak{v}$ to $\mathfrak{v}^c$ can be translated to a transition from $\mathfrak{w}$ to $\mathfrak{w}^c$. In particular, assuming that $v\in\mathfrak{v}$ makes the transition, the number of neighbors is given by $\bar{d}-\mathrm{deg}^{L_{\mathfrak{v}}}(v)$ again using the isomorphism between $L_{\mathfrak{v},\mathfrak{v}^c}$ and $L_{\mathfrak{w},\mathfrak{w}^c}$ there is a unique $w\in\mathfrak{w}$ with $\bar{d}-\mathrm{deg}^{L_{\mathfrak{v}}}(v)$ neighbors. Consequently, for any transition probability $p^{\triangle}_{k;\mathfrak{v},\mathfrak{u}}$ we can construct a transition from $\mathfrak{w}$ to some neighbor such that $p^{\triangle}_{k;\mathfrak{v},\mathfrak{u}} = p^{\triangle}_{k;\mathfrak{v},\mathfrak{u}}$. Therefore, we obtain $(p^{\triangle}_{k;\mathfrak{v},\mathfrak{u}})_{\mathfrak{u}\in\mathfrak{V}_k}=(p^{\triangle}_{k;\mathfrak{w},\mathfrak{u}})_{\mathfrak{u}\in\mathfrak{V}_k}$.\par 
	Since $L_{\mathfrak{v},\mathfrak{v}^c}$ defines the whole neighborhood of $\mathfrak{v}$ in $\mathfrak{L}_k$ the converse for $(p^{\triangle}_{k;\mathfrak{u},\mathfrak{v}})_{\mathfrak{u}\in\mathfrak{V}_k}=(p^{\triangle}_{k;\mathfrak{u},\mathfrak{w}})_{\mathfrak{u}\in\mathfrak{V}_k}$ is also true.\par
	The inverse direction is true since the transition probabilities $p^{\triangle}_{k;\mathfrak{v},\mathfrak{u}}$ uniquely define the number of particles in the neighborhood of any particle $v\in\mathfrak{v}$ and the inverse direction $p^{\triangle}_{k;\mathfrak{u},\mathfrak{v}}$ defines all neighbors of $\mathfrak{v}$ which can be created by displacing a single particle $v$. Consequently, the whole vectors $(p^{\triangle}_{k;\mathfrak{v},\mathfrak{u}})_{\mathfrak{u}\in\mathfrak{V}_k}$ and $(p^{\triangle}_{k;\mathfrak{u},\mathfrak{v}})_{\mathfrak{u}\in\mathfrak{V}_k}$ define all possible transitions and, hence, the bipartite graph $L_{\mathfrak{v},\mathfrak{v}^c}$. Consequently, if the vectors coincide for $\mathfrak{v},\mathfrak{w}\in\mathfrak{V}_k$, then, we obtain $L_{\mathfrak{v},\mathfrak{v}^c}\stackrel{\sim}{=} L_{\mathfrak{w},\mathfrak{w}^c}$.
\end{proof}
Hence, two configurations $\mathfrak{v},\mathfrak{w}$ which satisfy  $L_{\mathfrak{v},\mathfrak{v}^c}\stackrel{\sim}{=} L_{\mathfrak{w},\mathfrak{w}^c}$ are seen as identical when it comes to transitions for the Markov chain $\mathfrak{S}_k$. Additionally, by defining the equivalence relation $\mathfrak{v}\sim \mathfrak{w}$ if and only if $L_{\mathfrak{v},\mathfrak{v}^c}\stackrel{\sim}{=} L_{\mathfrak{w},\mathfrak{w}^c}$ and using Lemma \ref{lem:isom_of_bipartites_implies_same_transition_proba} as well as Proposition \ref{prop:isom_of_bipartites_implies_same_transition_vect} we find that for a fixed $\mathfrak{v}\in\mathfrak{V}_k$ and $\mathfrak{w}\in\mathfrak{V}_k$ such that $L_{\mathfrak{v},\mathfrak{v}^c}\stackrel{\sim}{=} L_{\mathfrak{w},\mathfrak{w}^c}$ we have the identity $|\{\mathfrak{u}\in\mathfrak{V}_k|\mathfrak{u}\sim \mathfrak{v},\;\langle \mathfrak{u}, \mathfrak{v} \rangle\in\mathfrak{E}_k \}| = |\{\mathfrak{u}'\in\mathfrak{V}_k|\mathfrak{u}'\sim \mathfrak{w},\;\langle \mathfrak{u}', \mathfrak{w} \rangle\in\mathfrak{E}_k \}|$ and there is a bijection $\Phi:\{\mathfrak{u}\in\mathfrak{V}_k|\mathfrak{u}\sim \mathfrak{v},\;\langle \mathfrak{u}, \mathfrak{v} \rangle\in\mathfrak{E}_k \} \to \{\mathfrak{u}'\in\mathfrak{V}_k|\mathfrak{u}'\sim \mathfrak{w},\;\langle \mathfrak{u}', \mathfrak{w} \rangle\in\mathfrak{E}_k \}$ such that $ p^{\triangle}_{k;\mathfrak{v},\mathfrak{u}}=p^{\triangle}_{k;\mathfrak{w},\Phi(\mathfrak{u})}$. This leads us to the realization that $\sum_{\mathfrak{u}\sim \mathfrak{v}} p^{\triangle}_{k;\mathfrak{v},\mathfrak{u}} =\sum_{\mathfrak{u}'\sim \mathfrak{w}} p^{\triangle}_{k;\mathfrak{w},\mathfrak{u}'}$ which forms the basis for the following central result.
\vspace{5pt}
\begin{tcolorbox}[boxsep=0pt,arc=0pt,colback=burgundy!15!white, frame empty]%%
	\begin{theorem}\label{thm:natural_lumping_of_L_k_for_S_k}
		Let $L=(V,E)$ be a $\bar{d}$-regular graph with $\bar{n}=|V|$ and $k\in\left\{1,\hdots,\bar{n}-1\right\}$. Denote by $\mathfrak{L}_k=(\mathfrak{V}_k,\mathfrak{E}_k)$ the $k$-particle graph and define for $\mathfrak{v},\mathfrak{w}\in\mathfrak{V}_k$ the equivalence relation $\mathfrak{v}\sim\mathfrak{w}$ if and only if $L_{\mathfrak{v},\mathfrak{v}^c}\stackrel{\sim}{=} L_{\mathfrak{w},\mathfrak{w}^c}$. For fixed $\mathfrak{v}$ define $[\mathfrak{v}_i]:=\{\mathfrak{u}\in\mathfrak{V}_k|\mathfrak{u}\sim\mathfrak{v}_i\}$ the equivalence class of $\mathfrak{v}_i$ and denote by $l$ the number of distinct equivalence classes. Then, the Markov chain $\mathfrak{S}_k$ is strongly lumpable with respect to the partition $\{[\mathfrak{v}_1],\hdots,[\mathfrak{v}_l]\}$. 
	\end{theorem}
\end{tcolorbox}
\begin{proof}
	We have to show that for any $\mathfrak{w}_1,\mathfrak{w}_2 \in [\mathfrak{v}_i]$ 
	\begin{equation*}
		\sum_{\mathfrak{u}\in [\mathfrak{v}_j]} p^{\triangle}_{k;\mathfrak{w}_1,\mathfrak{u}} = 	\sum_{\mathfrak{u}\in \mathfrak{u}\in [\mathfrak{v}_j]} p^{\triangle}_{k;\mathfrak{w}_2,\mathfrak{u}}.
	\end{equation*}
	The equality follows directly by Proposition \ref{prop:isom_of_bipartites_implies_same_transition_vect} and the following observation. For $\mathfrak{w}_1,\mathfrak{w}_2\in [\mathfrak{v}_i]$ and $\mathfrak{u}_1\in [\mathfrak{v}_j]$ with $\langle \mathfrak{w}_1,\mathfrak{u}_1\rangle\in\mathfrak{E}_k$ we have $\mathfrak{w}_1\triangle\mathfrak{u}_1=\{w,u\}$. Let $\Phi$ be the isomorphism between $L_{\mathfrak{w}_1,\mathfrak{w}_1^c}$ and $L_{\mathfrak{w}_2,\mathfrak{w}_2^c}$. There is a unique edge in $L_{\mathfrak{w}_2,\mathfrak{w}_2^c}$, namely $\langle \Phi(w),\Phi(u) \rangle$, $\mathrm{deg}^{L_{\mathfrak{w}_1}}(w)=\mathrm{deg}^{L_{\mathfrak{w}_2}}(\Phi(w))$ and for $\mathfrak{u}_2:= (\{\Phi(w_1)|w_1\in\mathfrak{w}_1\}\backslash \Phi(w))\cup\{\Phi(u)\}$ we have $\mathfrak{u}_1\sim \mathfrak{u}_2$ by construction. Consequently, for any summand in the first sum, we find a corresponding summand in the second sum and vice versa such that they are equal.    
\end{proof}
Lumpability gives rise to the possibility to consider the Markov chain on a smaller state space and in an aggregated form. While, usually, this makes it impossible to make local statements for example on the specific value of $\tilde{\pi}_k(\mathfrak{v})$ for some $\mathfrak{v}\in\mathfrak{V}_k$ about $\mathfrak{S}_k$ based on the lumped chain, the stronger form of lumpability implied by Lemma \ref{prop:isom_of_bipartites_implies_same_transition_vect} allows to formulate further deductions. A central one is the structure of the stationary distribution $\tilde{\pi}_k$ of $\mathfrak{S}_k$. 
\vspace{5pt}
\begin{tcolorbox}[boxsep=0pt,arc=0pt,colback=burgundy!15!white, frame empty]%%
	\begin{theorem}\label{thm:stationary_dist_level_sets_pi_k}
		Let $L=(V,E)$ be a $\bar{d}$-regular graph with $\bar{n}=|V|$ and $k\in\left\{1,\hdots,\bar{n}-1\right\}$. Denote by $\tilde{\pi}_k$ the stationary distribution of $\mathfrak{S}_k$. Then, for all equivalence classes $[\mathfrak{v}]$ under the equivalence relation $\sim$ defined in Theorem \ref{thm:natural_lumping_of_L_k_for_S_k} all $\mathfrak{v},\mathfrak{w}\in[\mathfrak{v}]$ satisfy the identity $\tilde{\pi}_k(\mathfrak{v})=\tilde{\pi}_k(\mathfrak{w})$.
	\end{theorem}
\end{tcolorbox}
We are going to present, first, an intuitive approach, which is based on the idea that by Proposition \ref{prop:isom_of_bipartites_implies_same_transition_vect} two equivalent vertices $\mathfrak{v},\mathfrak{w}\in\mathfrak{V}_k$ are "identical" when it comes to their respective probability in- and out-"flow" and the approach that the equality of the average $|[\bar{\mathfrak{v}}]|^{-1}\tilde{\pi}_k([\bar{\mathfrak{v}}])$ and $\tilde{\pi}_k(\mathfrak{w})$ for an arbitrary $\mathfrak{w}\in[\bar{\mathfrak{v}}]$ gives the claim we are looking for. The following calculations are only correct under the assumption that for any $\mathfrak{v},\mathfrak{w}\in[\bar{\mathfrak{v}}]$ we have for any equivalence class $[\bar{\mathfrak{u}}]$ the identity 
\begin{equation}\label{eq:heuristic_statement_equality_v_to_w_change}
	\sum_{\mathfrak{u}\in[\bar{\mathfrak{u}}]}\tilde{\pi}_k(\mathfrak{u})p^{\triangle}_{k;\mathfrak{u},\mathfrak{v}} = \sum_{\mathfrak{u}\in[\bar{\mathfrak{u}}]}\tilde{\pi}_k(\mathfrak{u})p^{\triangle}_{k;\mathfrak{u},\mathfrak{w}}.
\end{equation}  
While there are $\mathfrak{u},\mathfrak{u}'\in[\bar{\mathfrak{u}}]$ such that the equality $p^{\triangle}_{k;\mathfrak{u},\mathfrak{v}}=p^{\triangle}_{k;\mathfrak{u}',\mathfrak{w}}$ is satisfied we cannot make a similar claim about $\tilde{\pi}_k(\mathfrak{u})p^{\triangle}_{k;\mathfrak{u},\mathfrak{v}}$ and $\tilde{\pi}_k(\mathfrak{u}')p^{\triangle}_{k;\mathfrak{u}',\mathfrak{w}}$. This leads to a recursive statement where the truth of the claim for one equivalence class $[\bar{\mathfrak{v}}]$ depends on the truth of the claim for all neighboring equivalence classes $[\bar{\mathfrak{u}}]$. Assuming, then, \ref{eq:heuristic_statement_equality_v_to_w_change} is satisfied we obtain for a fixed $\mathfrak{w}\in[\bar{\mathfrak{v}}]$
\begin{align*}
	\tilde{\pi}_k([\bar{\mathfrak{v}}]) &=\sum_{[\bar{\mathfrak{u}}]\in\faktor{\mathfrak{V}_k}{\sim}}\tilde{\pi}_k([\bar{\mathfrak{u}}])\hat{p}_{[\bar{\mathfrak{u}}],[\bar{\mathfrak{v}}]}=\sum_{[\bar{\mathfrak{u}}]\in\faktor{\mathfrak{V}_k}{\sim}}\sum_{\mathfrak{u}\in[\bar{\mathfrak{u}}]}\tilde{\pi}_k(\mathfrak{u})\sum_{\mathfrak{v}\in[\bar{\mathfrak{v}}]} p^{\triangle}_{k,\mathfrak{u},\mathfrak{v}}\\
	&=\sum_{[\bar{\mathfrak{u}}]\in\faktor{\mathfrak{V}_k}{\sim}}\sum_{\mathfrak{u}\in[\bar{\mathfrak{u}}]}\sum_{\mathfrak{v}\in[\bar{\mathfrak{v}}]} \tilde{\pi}_k(\mathfrak{u})p^{\triangle}_{k,\mathfrak{u},\mathfrak{v}}=\sum_{[\bar{\mathfrak{u}}]\in\faktor{\mathfrak{V}_k}{\sim}}\sum_{\mathfrak{v}\in[\bar{\mathfrak{v}}]}\sum_{\mathfrak{u}\in[\bar{\mathfrak{u}}]} \tilde{\pi}_k(\mathfrak{u})p^{\triangle}_{k,\mathfrak{u},\mathfrak{v}}\\
	&\stackrel{\ref{eq:heuristic_statement_equality_v_to_w_change}}{=}\sum_{[\bar{\mathfrak{u}}]\in\faktor{\mathfrak{V}_k}{\sim}}\sum_{\mathfrak{v}\in[\bar{\mathfrak{v}}]}\sum_{\mathfrak{u}\in[\bar{\mathfrak{u}}]} \tilde{\pi}_k(\mathfrak{u})p^{\triangle}_{k,\mathfrak{u},\mathfrak{w}}=|[\bar{\mathfrak{v}}]|\sum_{\mathfrak{u}\in\mathfrak{V}_k} \tilde{\pi}_k(\mathfrak{u})p^{\triangle}_{k,\mathfrak{u},\mathfrak{w}}=|[\bar{\mathfrak{v}}]|\tilde{\pi}_k(\mathfrak{w}).
\end{align*}
This would lead to the claim of Theorem \ref{thm:stationary_dist_level_sets_pi_k} but the problem now lies in proving \ref{eq:heuristic_statement_equality_v_to_w_change}. This poses, again, a recursive problem in terms of the neighborhoods of each $\mathfrak{v}\in[\bar{\mathfrak{v}}]$ which is due to the missing information on the local structure of $\mathfrak{L}_k$ inaccessible. Indeed, we need a global perspective on $\mathfrak{L}_k$, which is based on cycles and their identification for equivalent vertices $\mathfrak{v},\mathfrak{w}$, where we denote the equivalence relation by $\sim$.
\begin{lemma}\label{lem:cycle_identifiation_on_equi_class}
	Let $L=(V,E)$ be a $\bar{d}$-regular graph and $\mathfrak{v},\mathfrak{w}\in\mathfrak{V}_k$. Define for $\mathfrak{v},\mathfrak{w}\in\mathfrak{V}_k$ the equivalence relation $\mathfrak{v}\sim\mathfrak{w}$ if and only if $L_{\mathfrak{v},\mathfrak{v}^c}\stackrel{\sim}{=} L_{\mathfrak{w},\mathfrak{w}^c}$. For fixed $\mathfrak{v}$ define $[\mathfrak{v}]:=\{\mathfrak{u}\in\mathfrak{V}_k|\mathfrak{u}\sim\mathfrak{v}\}$ the equivalence class of $\mathfrak{v}$. Let $\mathfrak{v},\mathfrak{w}\in[\bar{\mathfrak{v}}]$ for some $[\bar{\mathfrak{v}}]\in\faktor{\mathfrak{V}_k}{\sim}$ and $l\in\mathbb{N}$. Then for any cycle of length $l$ from $\mathfrak{v}$ to $\mathfrak{v}$ there is a cycle from $\mathfrak{w}$ to $\mathfrak{w}$ of length $l$. Additionally, the number of distinct cycles from $\mathfrak{v}$ to $\mathfrak{v}$ equals the number of distinct cycles from $\mathfrak{w}$ to $\mathfrak{w}$. 
\end{lemma}
\begin{proof}
	The proof works constructively, based on the fact that for any neighbor $\mathfrak{u}$ of $\mathfrak{v}$ we can find a neighbor $\hat{\mathfrak{u}}$ of $\mathfrak{w}$ such that $L_{\mathfrak{u},\mathfrak{u}^c}\stackrel{\sim}{=}L_{\hat{\mathfrak{u}},\hat{\mathfrak{u}}^c}$. This allows us to iteratively construct a cycle from $\mathfrak{w}$ to $\mathfrak{w}$ based on a cycle from $\mathfrak{v}$ to $\mathfrak{v}$.\par
	For $l\in\mathbb{N}$ denote by $\phi_{\mathfrak{v}}$ a cycle from $\mathfrak{v}$ to $\mathfrak{v}$. As mentioned in the introduction, we find to $\phi_{\mathfrak{v}}(2)$ a neighbor $\mathfrak{u}$ of $\mathfrak{w}$ such that $L_{\phi_{\mathfrak{v}}(2),\phi_{\mathfrak{v}}(2)^c}\stackrel{\sim}{=}L_{\mathfrak{u},\mathfrak{u}^c}$ by replacing $w\in\mathfrak{w}$ by $u\in\mathfrak{w}^c$ where $w$ is the image of $v\in\mathfrak{v}$ and $u$ the image of $v'\in\mathfrak{v}^c$ under the isomorphism given by $L_{\mathfrak{v},\mathfrak{v}^c}\stackrel{\sim}{=}L_{\mathfrak{w},\mathfrak{w}^c}$ and $\mathfrak{v}\triangle\phi_{\mathfrak{v}}(2)=\{v,v'\}$. We call $\phi_{\mathfrak{w}}(1):=\mathfrak{w}$ and $\phi_{\mathfrak{w}}(2):=\mathfrak{u}$. Restarting the same procedure for $\phi_{\mathfrak{v}}(2)$ and $\phi_{\mathfrak{v}}(3)$ in combination with $\phi_{\mathfrak{w}}(2)$ we obtain iteratively a cycle from $\mathfrak{w}$ to $\mathfrak{w}$ and this cycle has length $l$ since otherwise there is an index $l'<l$ such that $\phi_{\mathfrak{w}}(l')=\mathfrak{w}$ and applying the previous construction to $\phi_{\mathfrak{w}}(l'-1)$ leads to $\phi_{\mathfrak{v}}(l')=\mathfrak{v}$ which is a contradiction.\par
	By the previous construction there are at least as many cycles from $\mathfrak{w}$ to $\mathfrak{w}$ as are from $\mathfrak{v}$ to $\mathfrak{v}$. But by exchanging the roles of $\mathfrak{v}$ and $\mathfrak{w}$, which is possible due to the symmetry of the equivalence relation, we obtain also the inverse sense of the inequality such that there are as many cycles from $\mathfrak{w}$ to $\mathfrak{w}$ as are from $\mathfrak{v}$ to $\mathfrak{v}$. 
\end{proof}
Based on this geometric property of $\mathfrak{L}_k$ we can analyze the stationary distribution of $\mathfrak{S}_k$ as discussed in Theorem \ref{thm:stationary_dist_level_sets_pi_k} using first return times.

==> chapters/kPG_conc.tex <==
In this first Part reviewed some basic definitions from graph and set theory as well as established in the beginning some results, in particular with a focus on sub-graphs and their role (in regular graphs). This allowed us to define the central graph theoretical object of this work, the kPG $\mathfrak{L}_k$ associated to an underlying graph $L$, as defined in Definition \ref{def:mathfrak_L_k}. We managed to formulate and proof several properties of $\mathfrak{L}_k$ on connectivtiy, the combinatorial properties, the degree sequence as well as the automorphism group, always motivated and with the application in mind, which we will discuss at length in Part \ref{part:social_net_dyna}. Hence, instead of an extensive Outlook which cannot be complete in any sens, we keep it short and let the graph theory proficient reader decide, which of the immense number of open problems they want to tackle.  

==> chapters/kPG_marked_particles.tex <==
So far, we have analyzed the structure of $\mathfrak{L}_k$ if we consider simply subsets of $V$ of size $k$. This can be seen as indistinguishable particles and we record the configurations of the particles as unordered sets in the graph $\mathfrak{L}_k$. The problem becomes more involved as soon as we make the particles distinguishable. We can, then, differentiate the particles by names or give them numbers from $1$ to $k$. This leads to a natural vertex set, which is no longer $\mathfrak{V}_k$ but $V^k$. The discussion in \cite{WILSON197486} is the basis for what follows. For $\bar{v}\in V^k$ with $\bar{v}=(\bar{v}_1,\hdots,\bar{v}_k)$ we can interpret the entry $\bar{v}_i$ as the position of particle $i$ in $L$. Note that now configurations which are permutations of one another are distinguishable. A relevant example, which shows a possible application of marked particles on some finite graph, is the $15$-puzzle. This puzzle consist of a quadratic box which can fit $16$ quadratic tiles of adequate size and $15$ small enumerated quadratic tiles which correspond to this size carrying numbers $1$ to $15$. The game then consists in ordering the tiles row by row only by sliding one tile at the time using the remaining free slot, the first row containing the numbers $1$ to $4$, the second one the numbers $5$ to $8$ and so on. One can wonder about the existence of a solution to this task depending on the initial configuration of the tiles. Indeed, this example was already of interest for the authors of \cite{Greenwell1974} and it arises now naturally as a state space in the context of interacting particles.\par
We consider a simple connected graph $L=(V,E)$ as well as $k$ occupied sites $\{v_1,\hdots,v_k\}\subset V$. For $t\geq 0$ one of the occupied sides is chosen and the occupant moves to an adjacent side uniformly chosen among the free sides. If no free sides are available the configuration remains the same.  \par
Consequently, we can associate the dynamics with exclusion process $\eta=(\eta_t)_{t\in\mathbb{N}}$ on $L$. We reformulate the exclusion process on $L$ as a Markov chain on the a sub-graph of the Hamming graph.\par
Consider the following sub-graph of the Hamming graph $\mathcal{H}(\bar{n},k)=(V_{\mathcal{H}},E_{\mathcal{H}})$ and its vertex set
\begin{equation}\label{eq:exclusive_vertex_set}
	V_{\mathcal{H}} := \{\mathrm{v}=(\mathrm{v}_1,\hdots,\mathrm{v}_k)\in \mathrm{V}^k | \forall i,j\in\{1,\hdots,k\}, i\neq j: \mathrm{v}_i \neq \mathrm{v}_j\}.
\end{equation}
Due to fact that no two entries of any vector may have the same value and, therefore, any vertex in $V_{\mathcal{H}}$ represents a subset of size $k$ of $V$, we can conclude by the same reasoning as for $\mathfrak{V}_k$ that $V_{\mathcal{H}}$ is the correct choice to capture the configurations of the exclusion process. On the other hand, the edge set of $\mathcal{H}(\bar{n},k)$ is too large, since it does not take into consideration the structure of $L$, or, it corresponds to the case where $L$ is the complete graph. Thus, we have to make the following restriction to the edge set and arrive at
\begin{equation*}
	\mathfrak{E}_k^{(\mathfrak{m})} := \{\langle v,w\rangle\in E_{\mathcal{H}} | \exists ! i,\; 1\leq i\leq k: v_i \neq w_i,\; v_j = w_j\forall j\neq i,\; \langle v_i, w_i \rangle \in E \}.
\end{equation*}
We write $\mathfrak{V}_k^{(\mathfrak{m})}:=V_{\mathcal{H}}$ and denote by $\mathfrak{L}_k^{(\mathfrak{m})} := (\mathfrak{V}_k^{(\mathfrak{m})}, \mathfrak{E}_k^{(\mathfrak{m})})$ the marked kPG associated to $L$. The graph $\mathfrak{L}_k^{(\mathfrak{m})}$ can, hence, be understood as the state space of a particle system where a transition to a different configuration corresponds to the displacement of exactly one of the $k$ particles, each particle having a distinguishable mark. \par
To construct the graph representing the state space of a $k$-particle exclusion process with marked particles we remove all nodes from $\mathcal{H}(\bar{n},k)$ for which two coordinates coincide. Naturally all edges to which such a point is incident are also being removed. For $v\in \mathfrak{V}_k^{(\mathfrak{m})}$ we denote by $\mathrm{deg}_k^{(\mathfrak{m})}(v)$ its degree in $\mathfrak{L}_k^{(\mathfrak{m})}$.\par 
Some properties of $\mathfrak{L}_k^{(\mathfrak{m})}$ may be deduced from combinatorial considerations.
\begin{lemma}\label{lem:even_degree}
	The graph $\mathfrak{L}_k^{(\mathfrak{m})}$ has the following properties.
	\begin{itemize}
		\item The vertex set $\mathfrak{V}_k^{(\mathfrak{m})}$ has size $|\mathfrak{V}_k^{(\mathfrak{m})}|=\dfrac{\bar{n}!}{(\bar{n}-k)!}$
		\item For $\mathrm{v}\in \mathfrak{V}_k^{(\mathfrak{m})}$ denote by $L_{\mathrm{v}}$ the vertex induced subgraph of $\mathrm{v}$ in $L$. Then, the degree of $\mathrm{v}$ in $\mathfrak{L}_k^{(\mathfrak{m})}$ is given by $\mathrm{deg}_k^{(\mathfrak{m})}(\mathrm{v})=\sum_{i=1}^k\mathrm{deg}(v_i)-\mathrm{deg}^{L_{\mathrm{v}}}(v_i)$.
	\end{itemize}
\end{lemma}
\begin{proof}
	Since every vertex $\mathfrak{v}\in \mathfrak{V}_k^{(\mathfrak{m})}$ may be seen as a word of length $k$ constructed from an alphabet of length $\bar{n}>k$ where each letter may be used at most once, the property 
	\begin{equation*}
		|\mathfrak{V}_k^{(\mathfrak{m})}|=\dfrac{\bar{n}!}{(\bar{n}-k)!}
	\end{equation*} 
	follows from basic combinatorial considerations on drawing without replacement.\\
	To respect the geometry of $L$, two configurations can only be neighbors if the entries which differ are connected by an edge in $L$. Hence, any $v\in\mathrm{v}$ contributes $\mathrm{deg}(v)$ to the overall degree of $\mathrm{deg}_k^{(\mathfrak{m})}(\mathrm{v})$ when we do not take into account that at most one particle may occupy any vertex in $L$. Therefore, all $k$-tuples $\mathfrak{v}\in V^k$ with multiple identical entries are removed from $V^k$ to construct $\mathfrak{V}_k^{(\mathfrak{m})}$ and each vertex $\mathfrak{w}\in \mathfrak{V}_k^{(\mathfrak{m})}$ loses all such neighbors $\mathfrak{v}$. Therefore, for any $v\in\mathrm{v}$ we obtain its final contribution to $\mathrm{deg}_k^{(\mathfrak{m})}(\mathrm{v})$ given by $\mathrm{deg}(v)-\mathrm{deg}^{L_{\mathrm{v}}}(v)$. By summing over all $v\in\mathrm{v}$ we obtain $\mathrm{deg}^{L_{\mathfrak{v}}}=\sum_{i=1}^k\mathrm{deg}(v_i)-\mathrm{deg}^{L_{\mathrm{v}}}(v_i)$.
\end{proof}
Since marked particles are not the focus of this work, we only want to give a brief insight into the differences to unmarked particles. In particular, we no longer have connectedness of $\mathfrak{L}_k^{(\mathfrak{m})}$ if $L$ is connected. In fact, this has been shown in \cite{WILSON197486} where the author gives conditions on the graphs for which connectedness follows and we can use this result due to an isomorphism which we establish in Proposition \ref{prop:Hkr_connected}.
\begin{proposition}\label{prop:Hkr_connected}
	Let $k=\bar{n}-1$. Then $\mathfrak{L}_k^{(\mathfrak{m})}\stackrel{\sim}{=}\mathrm{puz}( L )$, as defined in \cite{WILSON197486}, and is therefore connected if and only if $\mathrm{puz}( L )$ is connected.
\end{proposition}
\begin{proof}
	The existence of an isomorphism follows directly by the construction of the two objects $\mathfrak{L}_k^{(\mathfrak{m})}$ and $\mathrm{puz}( L )$.
\end{proof}
We can, therefore, use the result found in \cite{WILSON197486} to make claims about the connectivity of not only $\mathfrak{L}_k^{(\mathfrak{m})}$ but also $\mathfrak{L}_{k'}^{(\mathfrak{m})}$ for all $k'<\bar{n}-1$.
\vspace{5pt}
\begin{tcolorbox}[boxsep=0pt,arc=0pt,colback=burntorange!25!white, frame empty]%%
	\begin{proposition}\label{prop:hkr_connected}
		Let $\mathrm{puz}( L )$ be connected. For $k\leq\bar{n}-1$ the graph $\mathfrak{L}_k^{(\mathfrak{m})}$ is connected. Otherwise $\mathfrak{L}_k^{(\mathfrak{m})}$ is the empty graph. 
	\end{proposition}
\end{tcolorbox}
\begin{proof}
	We start with the second case $k\geq \bar{n}$. Again the particle interpretation helps to make the point. Assume $k=\bar{n}$. Then all sides of $ L $ are occupied by particles. Hence any vertex in $\mathfrak{L}_k^{(\mathfrak{m})}$ is only a permutation of the set of all vertices in $ L $. Moreover no particle can move which implies that there are no edges between any vertices in $\mathfrak{L}_k^{(\mathfrak{m})}$. The graph $\mathfrak{L}_k^{(\mathfrak{m})}$ is therefore the empty graph. \par
	If $k>\bar{n}$ then we find by a direct combinatorial argument that any vertex in $V_k$ contains at least one entry twice. Hence by the deletion process in the construction of $\mathfrak{V}_k^{(\mathfrak{m})}$ we obtain $\mathfrak{V}_k^{(\mathfrak{m})}=\emptyset$.\par
	Let $k' < \bar{n}$ be the number of particles on $ L $. Denote by $d':= \bar{n}-1-k'$. Then for $k:= k'+ d'$ the graph $\mathfrak{L}_k^{(\mathfrak{m})}$ is connected by Lemma \ref{prop:Hkr_connected}. Let $\nu = (\nu_1,\hdots,\nu_{k'})$ and $\tilde{\nu} = (\tilde{\nu}_1,\hdots,\tilde{\nu}_{k'})$ be some configurations. Draw $d'$ unoccupied vertices 
	\begin{equation}
		\mu_1,\hdots,\mu_{d'}\in V \backslash \{\nu_1,\hdots,\nu_{k'}\}.
	\end{equation} 
	and $d'$ vertices
	\begin{equation}
		\tilde{\mu}_1,\hdots,\tilde{\mu}_{d'}\in V \backslash \{\tilde{\nu}_1,\hdots,\tilde{\nu}_{k'}\}.
	\end{equation} 
	Consider the configurations  $\nu^{d'}= (\nu_1,\hdots,\nu_{k'},\mu_1,\hdots,\mu_{d'})$ and $\tilde{\nu}^{d'} = (\tilde{\nu}_1,\hdots,\tilde{\nu}_{k'},\tilde{\mu}_1,\hdots,\tilde{\mu}_{d'})$. Then there is a path $\phi$ in $\mathfrak{L}_k^{(\mathfrak{m})}$ connecting $\nu^{d'}$ and $\tilde{\nu}^{d'}$, from which can be constructed a path in $H_{k'}^r$ by projection on the first $k'$ components. Hence $H_{k'}^r$ is connected.
\end{proof}    
Hence, for marked particles one could use $\mathfrak{L}_k^{(\mathfrak{m})}$ and its structure to represent configurations and their connections or characterize this family of graphs in itself combinatorically. We now turn to a probabilistic application of $\mathfrak{L}_k$ for which $\mathfrak{L}_k^{(\mathfrak{m})}$ is not suited since it enforces more constraints then necessary and desired. We consider the family of processes generalized exclusion processes which describe dynamical changes of configurations of unmarked particles which are mutually exclusive, i.e., a particle cannot move to an already occupied vertex.
